Slipstream: Ebb-and-Flow Consensus on a DAG with Fast Confirmation for UTXO Transactions

This paper introduces Slipstream, a Byzantine Fault Tolerance (BFT) protocol where nodes concurrently propose blocks to be added to a Directed Acyclic Graph (DAG) and aim to agree on block ordering. Slipstream offers two types of block orderings: an optimistic ordering, which is live and secure in a sleepy model under up to 50% Byzantine nodes, and a final ordering, which is a prefix of the optimistic ordering and ensures safety and liveness in an eventual lock-step synchronous model under up to 33% Byzantine nodes. Additionally, Slipstream integrates a payment system that allows for fast UTXO transaction confirmation independently of block ordering. Transactions are confirmed in three rounds during synchrony, and unconfirmed double spends are resolved in a novel way using the DAG structure.

==> Algorithm.tex <==
% % % % % % % % % % % % % % % % Chain-Switching% % % % % % % % % % % % % % % % % % % % 

\begin{algorithm}[pht]
\caption{$\textsc{ChainSwitching}()$ -- Procedure to switch the slot commitment chain.}
\label{alg: switch}
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\Input{Available DAG at instant $\langle s+1,1\rangle$, current commitment chain $\chain(\sigma_{s-1})=(\sigma_{-1}, \sigma_0, \ldots \sigma_{s-1})$}
\Output{Updated commitment chain $\chain(\theta_{s-1})$}

\BlankLine
$$

$\Sigma_{s-1}\gets $ set of all commitment chains up to slot $s-1$ in the buffer; including its own 
\tcp*{Find the supermajority prefix}

Let $\chain({\theta}_k)=(\theta_{-1}, \theta_0, \ldots, \theta_{k})$ be such that a supermajority, $(n+f)/2$, of the nodes have this prefix; $k$ is maximal \;

$\textsc{maxMajority}:=$ nodes having committed on the prefix $\chain({\theta}_k)$ during slot $s$ (at instant $\langle s, f+1 \rangle$) \;

$N_{s}:=$  number of nodes with blocks in slot $s$ (at instant $\langle s, f+1 \rangle$) in the buffer  \;

$consistentNodes := $ set of nodes that committed on $\sigma_{s-1}$ at $\langle s, f+2\rangle$  \;

\If{$|consistentNodes| < (N_{s}+1)/2$}
{   \tcp*{Switch commitment chain}
    \If{$\textsc{maxMajority} \neq \emptyset$}
    {
    leader := $\textsc{SelectLeader}(\textsc{maxMajority})$  \;
    }
    $\theta_{s-1}:=$ leader.commitment  \;
    \Return $\chain(\theta_{s-1})$ 
}
\Else{ 
        no update 
}
\end{algorithm}


% % % % % % % % % % % % % % % % Update-Available DAG % % % % % % % % % % % % % % % % % % % % 

\begin{algorithm}[pht]
\caption{$\textsc{UpdateDAG}()$ -- Procedure to update of the maintained DAG.}
\label{alg: updateDAG}
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\Input{Available DAG $D_a$, current commitment chain $\chain$, buffer}
\Output{Updated available DAG $D_a$}

\BlankLine
$\langle s, i\rangle:=$ current instant \;
$\sigma_{s-2}:= \chain_{s-2}$ \;
$Equivocator:=$ set of nodes that created an equivocation in slot $s-2$\;
\For{each block $B\in buffer\setminus D_a$}{
    \If{$ B.time \in \langle s, i-1 \rangle \cup \langle s-1, f+2 \rangle$}{
    $cone_s (B)$ := set of blocks $C$ in $cone(B)$ with $C.slot=s$ \;
    \If{ exists $C \in cone_s(B)$ such that $C.node \in Equivocator$ }{\textbf{continue}}
    \If{exists $C \in cone_s(B)$ such that $C.commit \neq  \sigma_{s-2}$}{\textbf{continue}} 
    $blockValid$ := \textsc{true} \;
    \For{each block $C \in cone(B)\setminus D_a$ not yet committed with $C.slot < s$}{
    $\textsc{ReachNumer}(C, \langle s, i\rangle):=$ number of nodes that created a block at slot $s$ from which one can reach $C$ (in the buffer)\;
    \If{$\textsc{ReachNumer}(C, \langle s, i\rangle)<i$}{
    $blockValid:=\textsc{false}$ \;
    \textbf{break}}
    }
    \If{$blockValid$}{
    $D_a:= D_a \cup cone(B)$} \;
    }
}
\end{algorithm}





% % % % % % % % % % % % % % % % Update-Chain % % % % % % % % % % % % % % % % % % % % 

\begin{algorithm}[pht]
\caption{$\textsc{UpdateChain}()$ -- Procedure to update the slot commitment chain.}
\label{alg: commitment}
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\Input{Available DAG $D_a$ at instant $\langle s+1, f+2\rangle$, current commitment chain $\chain(\sigma_{s-1})=(\sigma_{-1}, \sigma_0, \ldots \sigma_{s-1})$}
\Output{ Commitment $\sigma_s$ of slot $s$; updated commitment chain $\chain(\sigma_{s})$}

\BlankLine
%$Blocks_s :=$ the list of blocks in the available DAG created at or before slot $s$ and do not include a commitment contained in $\chain_{s-1}$ \;

%$orderedBlocks_s :=$ 

$Blocks_s \leftarrow \emptyset$ \tcp{list of blocks in the available DAG created at or before slot $s$ and do not include a commitment contained in $\chain_{s-1}$}

\For{each block $B\in D_a$}{

    \If{$B.commit \not \in \chain(\sigma_{s-1})$}{
        $Blocks_s:= \textsc{Append} (Blocks_s, B)$ \;
    }
}
$orderedBlocks_s:= \textsc{Order}(Blocks_s)$ \tcp{ordered list of blocks computed using an extension of the partial order induced by the available DAG $D_a$}
$\sigma_s = hash(\sigma_{s-1}, orderedBlocks_s)$ \;
$\chain(\sigma_{s}) = \textsc{Concat}(\chain(\sigma_{s-1}), \sigma_s) $ \;
\end{algorithm}


% % % % % % % % % % % % % % % % % Confirm-Transactions % % % % % % % % % % % % % % % % % % % 
\begin{algorithm}[pht]
\caption{$\textsc{ConfirmTransactions}()$ Update confirmed ledger.}
\label{alg: Confirmation}
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\Input{Confirmed ledger $\LOG_{\text{conf}}$}
\Output{Updated confirmed ledger $\LOG_{\text{conf}}$}

\BlankLine
$ApprovalSet_B$ := set of nodes in available DAG at slot $s+1$ or before that reference a supermajority of blocks approving a transaction $tx$ in block $B$, where $B.slot = s$ \; 

\For{$\forall B\in D$}{
    \For{each transaction $tx$ in $B$}{
            \If{all inputs of $tx$ are confirmed $\mathtt{and}$  $ |ApprovalSet_B|>(n+f)/2$} {
            Confirm transaction $tx$ \tcp*{Fast path} 
            Update $\LOG_{lc}$
          }
    }
}
\end{algorithm}


% % % % % % % % % % % % % % % % % Finalized slot % % % % % % % % % % % % % % % % % % % 


\begin{algorithm}[pht]
\caption{$\textsc{FinalizeSlot}()$ Update latest finalized slot index.}
\label{alg: Finality}
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}

\BlankLine
\Input{Available DAG at instant $\langle s, i\rangle$; latest slot index $s_{fin}$ of final commitment}
\Output{Updated slot index $s_{fin}$}
\For{each slot index $s'$ such that $s_{fin}+3\le s' \le s$}
{Set $S$ to be the latest blocks of distinct nodes in the available DAG created at slot $s'$\;
$setQC\gets \emptyset$  \tcp*{Set of QCs created at slot $s'$}
\For{each node $\mu$}{Set $qc$ be the latest quorum certificate reachable from the block in $S$ created by $\mu$\;
\If{$qc.slot=s'$}{$setQC\gets setQC\cup qc$}}
\If{$setQC$ contains $>(n-f)/2$ QCs that commit the same commitment}{$s_{fin}\gets s'-2$}
}
\end{algorithm}



% % % % % % % % % % % % % % % % % Finalized Ledger % % % % % % % % % % % % % % % % % % % 

\begin{algorithm}[t]
\caption{Procedures to update confirmed and final ledger.}
\label{alg: final ledger}
\scriptsize
\BlankLine
\Proc{\FinalizeTransactions()}{}
\tcp*{First add transactions that have certificates. This ensures fast-path confirmed transactions appear in the final ledger}
\For{$\forall B\in D(\sigma_{\tau_{i+1}-2})\setminus D(\sigma_{\tau_{i}-2})$}{
 \For{$\forall tx \in B.txs$} {
    \If{$\exists C\in D(\sigma_{\tau_{i+1}-1})$ s.t. $C$ is a TC for $tx$ in $B$} {
     \If{$tx$ has inputs in $\LOG_{\text{fin}}$} {
     \If{$tx\not \in \LOG_{\text{fin}}$} {
     \If{$tx$ is not conflicting with $\LOG_{\text{fin}}$}{
     $\LOG_{\text{fin}} \gets \LOG_{\text{fin}} \cup \{tx\}$\;  
     }
    }
    }
    }
    }    
}
\tcp*{Use total order to resolve conflicts}
\For{$\forall B\in D(\sigma_{\tau_{i+1}-2})\setminus D(\sigma_{\tau_{i}-2})$}{
 \For{$\forall tx \in B.txs$} {
    \If{$tx$ has inputs in $\LOG_{\text{fin}}$} {
     \If{$tx\not \in \LOG_{\text{fin}}$} {
     \If{$tx$ is not conflicting with $\LOG_{\text{fin}}$}{
     $\LOG_{\text{fin}} \gets \LOG_{\text{fin}} \cup \{tx\}$\;  
     }
    }
    }
    }    
}


\end{algorithm}

\begin{algorithm}[ht]
\scriptsize
\caption{Procedures to create a new block, update a slot commitment chain, and finalize a commitment.}
\label{alg: procedures CreateBlock UpdateChain FinalizeSlot}
%\SetKwInOut{Input}{Input}
%\SetKwInOut{Output}{Output}
%\Input{Available DAG at instant $\langle s, i\rangle$; latest commitment of the node $\sigma$ (for slot $s-2$ if $i<f+2$ or $s-1$ otherwise)}
%\Output{New block $B$}

\BlankLine

\Loc{}{
$\DAG\gets \{Genesis\}$ \tcp*{DAG maintained by the node}
$\chain\gets (0)$ \tcp*{Slot commitment chain adapted by the node}
$publicKey$ \tcp*{Public key of the node}
$s_{\text{final}}\gets 0$\tcp*{Slot index of the last final slot commitment}
$B_{\text{own}} \gets \{\}$ \tcp*{Last block created by the node}
}



\Func{\CreateBlock{}}{
$B\gets \{\}$\;
$B.refs\gets \textsc{Hash}(\textsc{Tips}())$ \tcp*{Hash references to all unreferenced blocks in $DAG$}
$B.txs\gets \textsc{Payload}()$ \tcp*{Subset of transactions}
$B.commit \gets \CurrentCommit()$\;
$B.time\gets \textsc{Now}()$ \tcp*{Current slot and instant indices}
$B.node \gets publicKey$ \;
$B.sign \gets \textsc{Sign}(B)$ \tcp*{Sign the content of block}
$B_{\text{own}}\gets B$\;
\Return $B$
}

\Func{\Tips{}}{
\Return $\{ B\in \DAG:\quad \nexists C\in \DAG: \Hash(B)\in C.refs \}$
}
\Func{\CurrentCommit{}}{
\Return $\chain.last$ \tcp*{Last element of chain}
}
\Func{\IsSupermajority{S}}{
\Return $|B.node: \ B\in S| \ge 2f+1$
}
\Proc{\UpdateChain{}}{
$\langle s+1,f+2 \rangle \gets \Now()$ \;
$\sigma_{s-1} \gets \CurrentCommit()$ \;
$r\gets \{\}$\;
$Blocks_{\le s} \gets \{B\in \DAG\setminus \DAG(\sigma_{s-1}) : \ B.slot \le s\}$\;
\For{$\forall B\in Blocks_{\le s}$}{
    $r\gets r || \Hash(B)$\;
}
%$orderedBlocks_s:= \textsc{Order}(Blocks_s)$ \tcp{ordered list of blocks computed using an extension of the partial order induced by the available DAG $D_a$}
$\sigma_{s} = \Hash(\sigma_{s-1}, r)$ \;
$\chain = \chain || \sigma_{s} $ \tcp*{Append the computed commitment to the end}
}
\Proc{\FinalizeBlocks{}}{
$\langle s,i \rangle \gets \Now()$ \;
\For{$\forall t \in [s_{\text{final}}+3, s]$}
{$\sigma_{t}\gets\chain[t]$\;
$Blocks_{=t}\gets \{B\in \DAG(\sigma_{t}) : \ B.slot = t\}$\;
$CC_{=t}\gets \{B\in Blocks_{=t}:\ B \text{ is a CC for $\sigma_{t-2}$} \}$\tcp*{ Commitment certificates from slot $t$ (Def.~\ref{def: quorum certificate})}
\If{$\IsSupermajority(CC_{=t})$}{
    $s_{\text{final}}\gets t-2$\;
}
}
}
\end{algorithm}

\begin{algorithm}[ht]
\scriptsize
\caption{Procedures to switch a slot commitment chain, and wake up.}
\label{alg: procedures CreateBlock UpdateChain FinalizeSlot}
%\SetKwInOut{Input}{Input}
%\SetKwInOut{Output}{Output}
%\Input{Available DAG at instant $\langle s, i\rangle$; latest commitment of the node $\sigma$ (for slot $s-2$ if $i<f+2$ or $s-1$ otherwise)}
%\Output{New block $B$}

\BlankLine

\Loc{}{
$\DAG\gets \{Genesis\}$ \tcp*{DAG maintained by the node}
$\chain\gets (0)$ \tcp*{Slot commitment chain adapted by the node}
$publicKey$ \tcp*{Public key of the node}
$s_{\text{final}}\gets 0$\tcp*{Slot index of the last final slot commitment}
$B_{\text{own}} \gets \{\}$ \tcp*{Last block created by the node}
}
\Proc{\ChainSwitching{}}{
    $\langle s+1, 1 \rangle \gets \Now()$\;
    $\sigma_{s-1}\gets \CurrentCommit()$\;
    $N_{\text{same}},N_{\text{total}} \gets 0$ \;
    \For{$node = \{1,2,\ldots, n\}$} {
     $B\gets \LastBlockFrom(node)$ \;
     \If{$B.time = \langle s, f+2\rangle$}{
     $N_{\text{total}}\gets N_{\text{total}}+1$\;
      \If{$B.commit = \sigma_{s-1}$}{
        $N_{\text{same}}\gets N_{\text{same}}+1$\;
        }
     }
    }    
    \If{$2N_{\text{same}} \le N_{\text{total}}$}{
        $leader \gets \Leader()$ \; 
        $B_{\text{leader}}\gets \LastBlockFrom(leader)$ \;
        $CC_{\text{leader}}\gets \LastCommitCertificate(B_{\text{leader}})$ \;
        $CC_{\text{own}}\gets \LastCommitCertificate(B_{\text{own}})$ \;
       \If{$CC_{\text{leader}}.slot \ge CC_{\text{own}}.slot$}{
        $\DAG \gets \DAG \cup cone(B_{\text{leader}})$\;
        $\chain \gets \chain(B_{\text{leader}}.commit)$ \;
        } 
    }   
}
\Proc{\WakeUp{}}{
    $\langle s+1, 1 \rangle \gets \Now()$\;
    $Multiset \gets \{\}$ \tcp*{Multiset of commitments}
    \For{$node = \{1,2,\ldots, n\}$} {
     $B\gets \LastBlockFrom(node)$ \;
     \If{$B.time = \langle s, f+2\rangle$}{    
      $Multiset\gets MultiSet \cup B.commit$ \;
     }     
    } 
    $\sigma_{s-1}\gets \Most(Multiset)$ \tcp*{Most present element} 
    $\chain \gets \chain(\sigma_{s-1})$ \;
    \For{$node = \{1,2,\ldots, n\}$} {
     $B\gets \LastBlockFrom(node)$ \;
     \If{$B.commit = \sigma_{s-1}$}{    
      $\DAG \gets \DAG \cup cone(B)$ \;
     }    
     }
}
\end{algorithm}

==> figures/futureAndPastCone.tex <==
%\tikzstyle{block_marking_red}[draw=red, thick, rounded corners=.1cm, inner sep=1pt]
\begin{figure}[t]
    \centering
\begin{tikzpicture}
% Block scheme
\def\xCoordinate{0.0}
\def\yCoordinate{0.0}
\def\yAdd{1.5}
\def\xAdd{0.75}
\def\innerSepar{-1.5}
\def\lineWidth{1.5}
\def\roundedCorners{1}
\def\opacityInternal{0.5}
\def\minHeight{20}
\def\minWidth{20}
\tikzstyle{block}=[draw, rectangle, minimum height=\minHeight pt, minimum width = \minWidth pt, text centered, rounded corners=\roundedCorners pt, draw=darkgray, font=\large]
\def\arrowStyle{-latex}
\node[block] (central_block) at (\xCoordinate,\yCoordinate) {$x$};
 \node [draw=red,opacity=\opacityInternal,rounded corners= \roundedCorners pt,line width = \lineWidth pt,
        inner sep=\innerSepar pt,fit=(central_block)] (red_central_block) {};
 \node [draw=blue, opacity=\opacityInternal, rounded corners =  \roundedCorners pt,line width = \lineWidth pt,
        inner sep=\innerSepar pt,fit=(red_central_block)] (blue_central_block) {};
        
\node[block] (blue_below_1_1) at (\xCoordinate-\xAdd,\yCoordinate-\yAdd) {};
 \node [draw=blue,opacity=\opacityInternal,rounded corners= \roundedCorners pt,line width = \lineWidth pt,
        inner sep=\innerSepar pt,fit=(blue_below_1_1)] (blue_blue_below_1_1) {};
 \draw[\arrowStyle] (blue_below_1_1) -- (central_block);  

\node[block] (blue_below_1_2) at (\xCoordinate+\xAdd,\yCoordinate-\yAdd) {};
 \node [draw=blue,opacity=\opacityInternal,rounded corners= \roundedCorners pt,line width = \lineWidth pt,
        inner sep=\innerSepar pt,fit=(blue_below_1_2)] (blue_blue_below_1_2) {};
 \draw[\arrowStyle] (blue_below_1_2) -- (central_block); 
 
 
 %\node[block] (blue_below_2_0) at (\xCoordinate-2*\xAdd,\yCoordinate-2*\yAdd) {};
 %\node [draw=blue,opacity=\opacityInternal,rounded corners= \roundedCorners pt,line width = \lineWidth pt,
 %       inner sep=\innerSepar pt,fit=(blue_below_2_0)] (blue_blue_below_2_0) {};
 %\draw[\arrowStyle] (blue_below_2_0) -- (blue_below_1_1); 
 
 \node[block] (blue_below_2_1) at (\xCoordinate,\yCoordinate-2*\yAdd) {};
 \node [draw=blue,opacity=\opacityInternal,rounded corners= \roundedCorners pt,line width = \lineWidth pt,
        inner sep=\innerSepar pt,fit=(blue_below_2_1)] (blue_blue_below_2_1) {};
 \draw[\arrowStyle] (blue_below_2_1) -- (blue_below_1_2); 
 \draw[\arrowStyle] (blue_below_2_1) -- (blue_below_1_1); 
 
 \node[block] (blue_below_2_2) at (\xCoordinate+2*\xAdd,\yCoordinate-2*\yAdd) {};
 \node [draw=blue,opacity=\opacityInternal,rounded corners= \roundedCorners pt,line width = \lineWidth pt,
        inner sep=\innerSepar pt,fit=(blue_below_2_2)] (blue_blue_below_2_2) {};
 \draw[\arrowStyle] (blue_below_2_2) -- (blue_below_1_2); 
 \draw[\arrowStyle, path fading = south]  (\xCoordinate,\yCoordinate-3*\yAdd) -- (blue_below_2_2) ; 
 \draw[\arrowStyle, path fading = south]  (\xCoordinate-3*\xAdd,\yCoordinate-3*\yAdd) -- (blue_below_2_1) ; 
 
 \draw[\arrowStyle, path fading = south]  (\xCoordinate+3*\xAdd,\yCoordinate-3*\yAdd) -- (blue_below_2_2) ; 
 
 
 \node[block] (red_above_1) at (\xCoordinate,\yCoordinate+\yAdd) {};
 \node [draw=red,opacity=\opacityInternal,rounded corners= \roundedCorners pt,line width = \lineWidth pt,
        inner sep=\innerSepar pt,fit=(red_above_1)] (red_red_above_1) {};
 \draw[\arrowStyle] (central_block) -- (red_above_1);

  \node[block] (red_above_2_1) at (\xCoordinate+\xAdd,\yCoordinate+2*\yAdd) {};
  \draw[\arrowStyle] (red_above_1) -- (red_above_2_1);
   \node [draw=red,opacity=\opacityInternal,rounded corners= \roundedCorners pt,line width = \lineWidth pt,
        inner sep=\innerSepar pt,fit=(red_above_2_1)] (red_red_above_2_1) {};
  
  \node[block] (red_above_2_2) at (\xCoordinate-\xAdd,\yCoordinate+2*\yAdd) {};
  \node [draw=red,opacity=\opacityInternal,rounded corners= \roundedCorners pt,line width = \lineWidth pt,
        inner sep=\innerSepar pt,fit=(red_above_2_2)] (red_red_above_2_2) {};
  \draw[\arrowStyle] (red_above_1) -- (red_above_2_2);
  
  
  \node[block] (red_above_3) at (\xCoordinate,\yCoordinate+3*\yAdd) {};
   \node [draw=red,opacity=\opacityInternal,rounded corners= \roundedCorners pt,line width = \lineWidth pt,
        inner sep=\innerSepar pt,fit=(red_above_3)] (red_red_above_3) {};
  \draw[\arrowStyle] (red_above_2_2) -- (red_above_3);
  \draw[\arrowStyle] (red_above_2_1) -- (red_above_3);

 \node[block] (red_above_3_0) at (\xCoordinate-2*\xAdd,\yCoordinate+3*\yAdd) {};
   \node [draw=red,opacity=\opacityInternal,rounded corners= \roundedCorners pt,line width = \lineWidth pt,
        inner sep=\innerSepar pt,fit=(red_above_3_0)] (red_red_above_3_0) {};
  \draw[\arrowStyle] (red_above_2_2) -- (red_above_3_0);
  \draw[\arrowStyle] (red_above_2_1) -- (red_above_3);
 \draw[\arrowStyle,path fading=north] (red_above_3) -- (\xCoordinate,\yCoordinate+4*\yAdd);
  \draw[\arrowStyle,path fading=north] (red_above_3_0) -- (\xCoordinate-\xAdd,\yCoordinate+4*\yAdd);
  \draw[\arrowStyle,path fading=north] (red_above_3_0) -- (\xCoordinate-2*\xAdd,\yCoordinate+4*\yAdd);
  

\node[block] (central_grey_left) at (\xCoordinate-2*\xAdd,\yCoordinate) {};
 \draw[\arrowStyle] (central_grey_left) -- (red_above_1);  
 
\node[block] (central_grey_right) at (\xCoordinate+2*\xAdd,\yCoordinate) {}; 

 \draw[\arrowStyle] (central_grey_right) -- (red_above_2_1);
 \draw[\arrowStyle] (blue_below_1_2) -- (central_grey_right);

 
 \node[block] (above_grey_1) at (\xCoordinate-3*\xAdd,\yCoordinate+\yAdd) {};
 \draw[\arrowStyle] (above_grey_1) -- (red_above_2_2);
\draw[\arrowStyle] (central_grey_left) -- (above_grey_1);
\draw[\arrowStyle] (blue_below_1_1) -- (central_grey_left);
\draw[\arrowStyle] (above_grey_1) -- (red_above_3_0);


 \node[block] (below_grey_1) at (\xCoordinate-3*\xAdd,\yCoordinate-\yAdd) {};
\draw[\arrowStyle] (below_grey_1) -- (above_grey_1);
\draw[\arrowStyle] (below_grey_1) -- (central_grey_left);
\draw[\arrowStyle] (blue_below_2_1) -- (below_grey_1);
\draw[\arrowStyle] (blue_below_2_2) -- (central_grey_right);

  \def\xCoordinate{0.0}
  \def\yCoordinate{\yAdd * 2/3}
  \def\x{3.0}
  \def\y{5.0}
  \def\R{\x+0.004}
  \def\yc{\y+0.02}
  \def\e{0.4}
  \def\opacityCones{0.2} 
  
  
  
  
  % blue future cone 1
  \node at (\xCoordinate-\x/2,\yCoordinate-\y*5/6)  {\color{blue} future  cone};
  \begin{scope}[rotate=0]
    \shade[right color=white,left color=blue,opacity=\opacityCones]
      (\xCoordinate-\x,\yCoordinate-\yc) arc (180:360:{\R} and \e) -- (\xCoordinate+\x,\yCoordinate-\yc) -- (\xCoordinate,\yCoordinate) -- cycle;
    \draw[fill=blue,opacity=\opacityCones]
      (\xCoordinate,\yCoordinate-\yc) circle ({\R} and \e);
    \draw[blue, dashed]
      (\xCoordinate-\x,\yCoordinate-\y) -- (\xCoordinate,\yCoordinate) -- (\xCoordinate+\x,\yCoordinate-\y);
    \draw[blue, dashed]
      (\xCoordinate,\yCoordinate-\yc) circle ({\R} and \e);
  \end{scope}
 
 
 
 \def\yCoordinate{-\yAdd * 2/3}
  \def\x{3.0}
  \def\y{6.6}
  \def\R{\x+0.004}
  \def\yc{\y+0.02}
  % red cone 2
   \node at (\xCoordinate+\x*1/2,\yCoordinate+\y*5/6)  {\color{red} past cone};
  \begin{scope}[rotate=0]
    \shade[left color=white, right color=red,opacity=\opacityCones]
    (\xCoordinate-\x,\yCoordinate+\yc) arc (180:360:{\R} and \e) -- (\xCoordinate+\x,\yCoordinate+\yc) -- (\xCoordinate,\yCoordinate) -- cycle;
     \draw[fill=red,opacity=0.3*\opacityCones]
      (\xCoordinate+0,\yCoordinate+\yc) circle ({\R} and \e);
    \draw[red, dashed]
      (\xCoordinate-\x,\yCoordinate+\y) -- (\xCoordinate,\yCoordinate) -- (\xCoordinate+\x,\yCoordinate+\y);
    \draw[red, dashed]
      (\xCoordinate,\yCoordinate+\yc) circle ({\R} and \e);
  \end{scope}
  
\node [single arrow,top  color=red, bottom color=blue,
single arrow head extend=3pt,transform shape, opacity = 2*\opacityCones, minimum height=280pt, text opacity=1, rotate = 270, anchor=west] 
at (\xCoordinate+\x*7/6,\yCoordinate+\y){time
};
 
\end{tikzpicture}
\caption{Future and past cones of a block $x$ in the block DAG \todo{Remove future cone}}
    \label{fig:conesInTangle}
\end{figure}
